Study of proton parton distribution functions at high x using ZEUS data

At large values of x the parton distribution functions (PDFs) of the proton are poorly constrained and there are considerable variations between different global fits. Data at such high x have already been published by the ZEUS Collaboration, but not yet used in PDF extractions. A technique for comparing predictions based on different PDF sets to the observed number of events in the ZEUS data is presented. It is applied to compare predictions from the most commonly used PDFs to published ZEUS data at high Bjorken x. A wide variation is found in the ability of the PDFs to predict the observed results. A scheme for including the ZEUS high-x data in future PDF extractions is discussed.

==> auth187_new.tex <==
     





%===================================================================
%
%  MEMBER NAME  AUTH183 (ZEUS)     M  TEX
%
%  JH.: transformed to a format, which is suited as input for
%       CONVERT, which automatically creates author-indices
%
%  Don't remove lines starting with a percent sign %,
%  CONVERT may need them urgently !
%  
%=====================================================================
                                                   %
\begin{center}
{                      \Large  The ZEUS Collaboration              }
\end{center}

{\small\raggedright


%  members:

I.~Abt$^{19}$, 
L.~Adamczyk$^{7}$, 
R. Aggarwal$^{3, b}$, 
V.~Aushev$^{17}$, 
O.~Behnke$^{9}$, 
U.~Behrens$^{9}$, 
A.~Bertolin$^{21}$, 
I.~Bloch$^{10}$, 
I.~Brock$^{2}$, 
N.H.~Brook$^{28, m}$, 
R.~Brugnera$^{22}$, 
A.~Bruni$^{1}$, 
P.J.~Bussey$^{11}$, 
A.~Caldwell$^{19}$, 
M.~Capua$^{4}$, 
C.D.~Catterall$^{32}$, 
J.~Chwastowski$^{6}$, 
J.~Ciborowski$^{29, o}$, 
R.~Ciesielski$^{9, d}$, 
A.M.~Cooper-Sarkar$^{20}$, 
M.~Corradi$^{1, a}$, 
R.K.~Dementiev$^{18}$, 
S.~Dusini$^{21}$, 
J.~Ferrando$^{9}$, 
B.~Foster$^{20, j}$, 
E.~Gallo$^{13, k}$, 
D.~Gangadharan$^{14}$, 
A.~Garfagnini$^{22}$, 
A.~Geiser$^{9}$, 
L.K.~Gladilin$^{18}$, 
Yu.A.~Golubkov$^{18}$, 
G.~Grzelak$^{29}$, 
C.~Gwenlan$^{20}$, 
D.~Hochman$^{31}$, 
N.Z.~Jomhari$^{9}$, 
I.~Kadenko$^{17}$, 
S.~Kananov$^{23}$, 
U.~Karshon$^{31}$, 
P.~Kaur$^{3, c}$, 
R.~Klanner$^{13}$, 
U.~Klein$^{9, e}$, 
I.A.~Korzhavina$^{18}$, 
N.~Kovalchuk$^{13}$, 
H.~Kowalski$^{9}$, 
O.~Kuprash$^{9, f}$, 
M.~Kuze$^{25}$, 
B.B.~Levchenko$^{18}$, 
A.~Levy$^{23}$, 
B.~L\"ohr$^{9}$, 
A.~Longhin$^{22}$, 
O.Yu.~Lukina$^{18}$, 
I.~Makarenko$^{9}$, 
J.~Malka$^{9, g}$, 
S.~Masciocchi$^{12, i}$, 
K.~Nagano$^{15}$, 
J.D.~Nam$^{24}$, 
J.~Onderwaater$^{14, l}$, 
Yu.~Onishchuk$^{17}$, 
E.~Paul$^{2}$, 
I.~Pidhurskyi$^{17}$, 
A.~Polini$^{1}$, 
M.~Przybycie\'n$^{7}$, 
A.~Quintero$^{24}$, 
M.~Ruspa$^{27}$, 
D.H.~Saxon$^{11}$, 
U.~Schneekloth$^{9}$, 
T.~Sch\"orner-Sadenius$^{9}$, 
I.~Selyuzhenkov$^{12}$, 
M.~Shchedrolosiev$^{17}$, 
L.M.~Shcheglova$^{18}$, 
I.O.~Skillicorn$^{11}$, 
W.~S{\l}omi\'nski$^{8}$, 
A.~Solano$^{26}$, 
L.~Stanco$^{21}$, 
N.~Stefaniuk$^{9}$, 
P.~Stopa$^{6}$, 
B.~Surrow$^{24}$, 
J.~Sztuk-Dambietz$^{13, g}$, 
E.~Tassi$^{4}$, 
K.~Tokushuku$^{15}$, 
M.~Turcato$^{13, g}$, 
O.~Turkot$^{9}$, 
T.~Tymieniecka$^{30}$, 
A.~Verbytskyi$^{19}$, 
W.A.T.~Wan Abdullah$^{5}$, 
K.~Wichmann$^{9}$, 
M.~Wing$^{28, n}$, 
S.~Yamada$^{15}$, 
Y.~Yamazaki$^{16}$, 
A.F.~\.Zarnecki$^{29}$, 
L.~Zawiejski$^{6}$, 
O.~Zenaiev$^{9, h}$ 
\newpage

%       institutes:

{\setlength{\parskip}{0.4em}
\makebox[3ex]{$^{1}$}
\begin{minipage}[t]{14cm}
{\it INFN Bologna, Bologna, Italy}~$^{A}$

\end{minipage}

\makebox[3ex]{$^{2}$}
\begin{minipage}[t]{14cm}
{\it Physikalisches Institut der Universit\"at Bonn,
Bonn, Germany}~$^{B}$

\end{minipage}

\makebox[3ex]{$^{3}$}
\begin{minipage}[t]{14cm}
{\it Panjab University, Department of Physics, Chandigarh, India}

\end{minipage}

\makebox[3ex]{$^{4}$}
\begin{minipage}[t]{14cm}
{\it Calabria University,
Physics Department and INFN, Cosenza, Italy}~$^{A}$

\end{minipage}

\makebox[3ex]{$^{5}$}
\begin{minipage}[t]{14cm}
{\it National Centre for Particle Physics, Universiti Malaya, 50603 Kuala Lumpur, Malaysia}~$^{C}$

\end{minipage}

\makebox[3ex]{$^{6}$}
\begin{minipage}[t]{14cm}
{\it The Henryk Niewodniczanski Institute of Nuclear Physics, Polish Academy of \\
Sciences, Krakow, Poland}

\end{minipage}

\makebox[3ex]{$^{7}$}
\begin{minipage}[t]{14cm}
{\it AGH University of Science and Technology, Faculty of Physics and Applied Computer
Science, Krakow, Poland}

\end{minipage}

\makebox[3ex]{$^{8}$}
\begin{minipage}[t]{14cm}
{\it Department of Physics, Jagellonian University, Krakow, Poland}~$^{D}$

\end{minipage}

\makebox[3ex]{$^{9}$}
\begin{minipage}[t]{14cm}
{\it Deutsches Elektronen-Synchrotron DESY, Hamburg, Germany}

\end{minipage}

\makebox[3ex]{$^{10}$}
\begin{minipage}[t]{14cm}
{\it Deutsches Elektronen-Synchrotron DESY, Zeuthen, Germany}

\end{minipage}

\makebox[3ex]{$^{11}$}
\begin{minipage}[t]{14cm}
{\it School of Physics and Astronomy, University of Glasgow,
Glasgow, United Kingdom}~$^{E}$

\end{minipage}

\makebox[3ex]{$^{12}$}
\begin{minipage}[t]{14cm}
{\it GSI Helmholtzzentrum f\"{u}r Schwerionenforschung GmbH, Darmstadt, Germany}

\end{minipage}

\makebox[3ex]{$^{13}$}
\begin{minipage}[t]{14cm}
{\it Hamburg University, Institute of Experimental Physics, Hamburg,
Germany}~$^{F}$

\end{minipage}

\makebox[3ex]{$^{14}$}
\begin{minipage}[t]{14cm}
{\it Physikalisches Institut of the University of Heidelberg, Heidelberg, Germany}

\end{minipage}

\makebox[3ex]{$^{15}$}
\begin{minipage}[t]{14cm}
{\it Institute of Particle and Nuclear Studies, KEK,
Tsukuba, Japan}~$^{G}$

\end{minipage}

\makebox[3ex]{$^{16}$}
\begin{minipage}[t]{14cm}
{\it Department of Physics, Kobe University, Kobe, Japan}~$^{G}$

\end{minipage}

\makebox[3ex]{$^{17}$}
\begin{minipage}[t]{14cm}
{\it Department of Nuclear Physics, National Taras Shevchenko University of Kyiv, Kyiv, Ukraine}

\end{minipage}

\makebox[3ex]{$^{18}$}
\begin{minipage}[t]{14cm}
{\it Lomonosov Moscow State University, Skobeltsyn Institute of Nuclear Physics,
Moscow, Russia}

\end{minipage}

\makebox[3ex]{$^{19}$}
\begin{minipage}[t]{14cm}
{\it Max-Planck-Institut f\"ur Physik, M\"unchen, Germany}

\end{minipage}

\makebox[3ex]{$^{20}$}
\begin{minipage}[t]{14cm}
{\it Department of Physics, University of Oxford,
Oxford, United Kingdom}~$^{E}$

\end{minipage}

\makebox[3ex]{$^{21}$}
\begin{minipage}[t]{14cm}
{\it INFN Padova, Padova, Italy}~$^{A}$

\end{minipage}

\makebox[3ex]{$^{22}$}
\begin{minipage}[t]{14cm}
{\it Dipartimento di Fisica e Astronomia dell' Universit\`a and INFN,
Padova, Italy}~$^{A}$

\end{minipage}

\makebox[3ex]{$^{23}$}
\begin{minipage}[t]{14cm}
{\it Raymond and Beverly Sackler Faculty of Exact Sciences, School of Physics, \\
Tel Aviv University, Tel Aviv, Israel}~$^{H}$

\end{minipage}

\makebox[3ex]{$^{24}$}
\begin{minipage}[t]{14cm}
{\it Department of Physics, Temple University, Philadelphia, PA 19122, USA}~$^{I}$

\end{minipage}

\makebox[3ex]{$^{25}$}
\begin{minipage}[t]{14cm}
{\it Department of Physics, Tokyo Institute of Technology,
Tokyo, Japan}~$^{G}$

\end{minipage}

\makebox[3ex]{$^{26}$}
\begin{minipage}[t]{14cm}
{\it Universit\`a di Torino and INFN, Torino, Italy}~$^{A}$

\end{minipage}

\makebox[3ex]{$^{27}$}
\begin{minipage}[t]{14cm}
{\it Universit\`a del Piemonte Orientale, Novara, and INFN, Torino,
Italy}~$^{A}$

\end{minipage}

\makebox[3ex]{$^{28}$}
\begin{minipage}[t]{14cm}
{\it Physics and Astronomy Department, University College London,
London, United Kingdom}~$^{E}$

\end{minipage}

\makebox[3ex]{$^{29}$}
\begin{minipage}[t]{14cm}
{\it Faculty of Physics, University of Warsaw, Warsaw, Poland}

\end{minipage}

\makebox[3ex]{$^{30}$}
\begin{minipage}[t]{14cm}
{\it National Centre for Nuclear Research, Warsaw, Poland}

\end{minipage}

\makebox[3ex]{$^{31}$}
\begin{minipage}[t]{14cm}
{\it Department of Particle Physics and Astrophysics, Weizmann
Institute, Rehovot, Israel}

\end{minipage}

\makebox[3ex]{$^{32}$}
\begin{minipage}[t]{14cm}
{\it Department of Physics, York University, Ontario, Canada M3J 1P3}~$^{J}$

\end{minipage}

}

\vspace{3em}

%  references concerning institutes;

{\setlength{\parskip}{0.4em}\raggedright
\makebox[3ex]{$^{ A}$}
\begin{minipage}[t]{14cm}
 supported by the Italian National Institute for Nuclear Physics (INFN) \
\end{minipage}

\makebox[3ex]{$^{ B}$}
\begin{minipage}[t]{14cm}
 supported by the German Federal Ministry for Education and Research (BMBF), under
 contract No.\ 05 H09PDF\
\end{minipage}

\makebox[3ex]{$^{ C}$}
\begin{minipage}[t]{14cm}
 supported by HIR grant UM.C/625/1/HIR/149 and UMRG grants RU006-2013, RP012A-13AFR and RP012B-13AFR from
 Universiti Malaya, and ERGS grant ER004-2012A from the Ministry of Education, Malaysia\
\end{minipage}

\makebox[3ex]{$^{ D}$}
\begin{minipage}[t]{14cm}
supported by the Polish National Science Centre (NCN) grant no.\ DEC-2014/13/B/ST2/02486
\end{minipage}

\makebox[3ex]{$^{ E}$}
\begin{minipage}[t]{14cm}
 supported by the Science and Technology Facilities Council, UK\
\end{minipage}

\makebox[3ex]{$^{ F}$}
\begin{minipage}[t]{14cm}
 supported by the German Federal Ministry for Education and Research (BMBF), under
 contract No.\ 05h09GUF, and the SFB 676 of the Deutsche Forschungsgemeinschaft (DFG) \
\end{minipage}

\makebox[3ex]{$^{ G}$}
\begin{minipage}[t]{14cm}
 supported by the Japanese Ministry of Education, Culture, Sports, Science and Technology
 (MEXT) and its grants for Scientific Research\
\end{minipage}

\makebox[3ex]{$^{ H}$}
\begin{minipage}[t]{14cm}
 supported by the Israel Science Foundation\
\end{minipage}

\makebox[3ex]{$^{ I}$}
\begin{minipage}[t]{14cm}
 supported in part by the Office of Nuclear Physics within the U.S.\ DOE Office of Science
\end{minipage}

\makebox[3ex]{$^{ J}$}
\begin{minipage}[t]{14cm}
 supported by the Natural Sciences and Engineering Research Council of Canada (NSERC) \
\end{minipage}

}

\pagebreak[4]
{\setlength{\parskip}{0.4em}

%  references concerning members;

\makebox[3ex]{$^{ a}$}
\begin{minipage}[t]{14cm}
now at INFN Roma, Italy\
\end{minipage}

\makebox[3ex]{$^{ b}$}
\begin{minipage}[t]{14cm}
now at DST-Inspire Faculty, Department of Technology, SPPU, India\
\end{minipage}

\makebox[3ex]{$^{ c}$}
\begin{minipage}[t]{14cm}
now at Sant Longowal Institute of Engineering and Technology, Longowal, Punjab, India\
\end{minipage}

\makebox[3ex]{$^{ d}$}
\begin{minipage}[t]{14cm}
now at Rockefeller University, New York, NY 10065, USA\
\end{minipage}

\makebox[3ex]{$^{ e}$}
\begin{minipage}[t]{14cm}
now at University of Liverpool, United Kingdom\
\end{minipage}

\makebox[3ex]{$^{ f}$}
\begin{minipage}[t]{14cm}
now at University of Freiburg, Freiburg, Germany\
\end{minipage}

\makebox[3ex]{$^{ g}$}
\begin{minipage}[t]{14cm}
now at European X-ray Free-Electron Laser facility GmbH, Hamburg, Germany\
\end{minipage}

\makebox[3ex]{$^{ h}$}
\begin{minipage}[t]{14cm}
now at Hamburg University, Hamburg, Germany\
\end{minipage}

\makebox[3ex]{$^{ i}$}
\begin{minipage}[t]{14cm}
also at Physikalisches Institut of the University of Heidelberg, Heidelberg,  Germany\
\end{minipage}

\makebox[3ex]{$^{ j}$}
\begin{minipage}[t]{14cm}
also at DESY and University of Hamburg\
\end{minipage}

\makebox[3ex]{$^{ k}$}
\begin{minipage}[t]{14cm}
also at DESY\
\end{minipage}

\makebox[3ex]{$^{ l}$}
\begin{minipage}[t]{14cm}
also at GSI Helmholtzzentrum f\"{u}r Schwerionenforschung GmbH, Darmstadt, Germany\
\end{minipage}

\makebox[3ex]{$^{ m}$}
\begin{minipage}[t]{14cm}
now at University of Bath, United Kingdom\
\end{minipage}

\makebox[3ex]{$^{ n}$}
\begin{minipage}[t]{14cm}
also supported by DESY\
\end{minipage}

\makebox[3ex]{$^{ o}$}
\begin{minipage}[t]{14cm}
also at Lodz University, Poland\
\end{minipage}

}


}


==> t_Transfer_matrix <==
#!/bin/sh
#
#       To run LaTeX and BibTeX on a given LaTeX source file
#       -> Part of LaTeX4zeus, added in version pre-1.0 <-
#
#       Author: I. Brock, University of Bonn, May 2011
#               Bug reports etc. to brock@physik.uni-bonn.de
#
#-------------------------------------------------------------------------------
#   Usage information
#-------------------------------------------------------------------------------
usage() {
cat <<EOF
Usage: $0 [options]

OPTIONS:
 -q   quiet: i.e. no output to terminal
 -m   medium: output of first latex command, bibtex
      and dvips to terminal (default)
 -v   verbose: all output to terminal
 -a   to use arXiV version
 -d   to use latex/dvips instead of pdflatex
 -p   to use pdflatex instead of latex
 -h   to use hugelatex instead of latex (if available)
 -b   do not run BiBTeX - final version that has bbl already

 Note that all command output is collected in file ${prog}.l4l,
 independent of the choice of options.
EOF
}

#-------------------------------------------------------------------------------
#   Functions to run LaTeX/PDFLaTeX and BiBTeX
#-------------------------------------------------------------------------------
runlatex () {
    echo " ==> Calling LaTeX"
    echo "" >> ${prog}.l4l
    echo " ==> Calling LaTeX" >> ${prog}.l4l
    echo " -----------------" >> ${prog}.l4l
    $ltcom ${prog}.tex | tee -a ${prog}.l4l 2> $rdct ||\
     (echo " First LaTeX run failed (see transcript file ${prog}.log)"; exit 1)
    echo "" >> ${prog}.l4l
    echo " ==> LaTeX log file (call $run)" >> ${prog}.l4l
    echo " ---------------------------" >> ${prog}.l4l
    cat ${prog}.log >> ${prog}.l4l
}

runbibtex() {
    echo " ==> Calling BibTeX"
    echo "" >> ${prog}.l4l
    echo " ==> Calling BibTeX" >> ${prog}.l4l
    echo " ------------------" >> ${prog}.l4l
    bibtex ${prog} | tee -a ${prog}.l4l 2> $rdctb ||\
     (echo " BiBTeX run failed (see transcript file ${prog}.blg)"; exit 1)
    echo "" >> ${prog}.l4l
    echo " ==> BiBTeX log file" >> ${prog}.l4l
    echo " -------------------" >> ${prog}.l4l
    cat ${prog}.blg >> ${prog}.l4l
}

rundvips() {
    echo " ==> Calling dvips"
    echo "" >> ${prog}.l4l
    echo " ==> Calling dvips" >> ${prog}.l4l
    echo " -----------------" >> ${prog}.l4l
    dvips -t a4 ${prog}.dvi -o | tee -a ${prog}.l4l 2> $rdctd
    sta=$?
    if [ $sta -ne 0 ]; then
        echo " dvips failed - status" $sta
        echo " dvips failed - status" $sta >> ${prog}.log
        exit
    fi
}

#-------------------------------------------------------------------------------
#   Check arguments
#-------------------------------------------------------------------------------
prog='Transfer_matrix'
#
rdct1='/dev/tty'
rdctb='/dev/tty'
rdct2='/dev/null'
rdct3='/dev/null'
rdctd='/dev/tty'
ltcom='latex'
#------------------------------------------------------------------------------
# If BiBTeX directory does not exist, turn off bibtex
#------------------------------------------------------------------------------
if [ -d BiBTeX -o -h BiBTeX ]; then
    runbibtex=1
else
    runbibtex=0
fi
#
while getopts bBqQmMdDpPvVhH opt; do
    case $opt in
        q|Q)
            rdct1='/dev/null'
            rdctb='/dev/null'
            rdctd='/dev/null'
            ;;
        m|M)
            ;;
        v|V)
            rdct2='/dev/tty'
            rdct3='/dev/tty'
            shift
            ;;
        b|B)
            runbibtex=0
            ;;
        d|D)
            ltcom=latex
            shift
            ;;
        p|P)
            ltcom=pdflatex
            shift
            ;;
        h|H)
            which hugelatex 2>/dev/null
            check=$?
            if [ $check -eq 0 ]; then
                ltcom='hugelatex'
            else
                echo "WARNING: hugelatex not available. Using latex."
                ltcom='latex'
            fi
            shift
            ;;
        ?)
            usage
            exit 1
            ;;
    esac
done

#-------------------------------------------------------------------------------
#   First latex run
#-------------------------------------------------------------------------------
touch ${prog}.l4l
run=1
rdct=$rdct1
runlatex
#-------------------------------------------------------------------------------
#   bibtex run
#-------------------------------------------------------------------------------
if [ $runbibtex -eq 1 ]; then
    runbibtex
fi
#-------------------------------------------------------------------------------
#   Second latex run
#-------------------------------------------------------------------------------
run=2
rdct=$rdct2
runlatex
#-------------------------------------------------------------------------------
#   Third latex run
#-------------------------------------------------------------------------------
run=3
rdct=$rdct3
runlatex
#-------------------------------------------------------------------------------
#   Finally call dvips if we are running LaTeX
#-------------------------------------------------------------------------------
if [ $ltcom = "latex" ]; then
    rundvips
fi
exit

